Confidence-Based Response Abstinence: Improving LLM Trustworthiness via Activation-Based Uncertainty Estimation

We propose a method for confidence estimation in retrieval-augmented generation (RAG) systems that aligns closely with the correctness of large language model (LLM) outputs. Confidence estimation is especially critical in high-stakes domains such as finance and healthcare, where the cost of an incorrect answer outweighs that of not answering the question. Our approach extends prior uncertainty quantification methods by leveraging raw feed-forward network (FFN) activations as auto-regressive signals, avoiding the information loss inherent in token logits and probabilities after projection and softmax normalization. We model confidence prediction as a sequence classification task, and regularize training with a Huber loss term to improve robustness against noisy supervision. Applied in a real-world financial industry customer-support setting with complex knowledge bases, our method outperforms strong baselines and maintains high accuracy under strict latency constraints. Experiments on Llama 3.1 8B model show that using activations from only the 16th layer preserves accuracy while reducing response latency. Our results demonstrate that activation-based confidence modeling offers a scalable, architecture-aware path toward trustworthy RAG deployment.

==> introduction.tex <==
\section{Introduction}

\dl{Introduction is probably the most important section which sets a tone of like/dislike for readers before reading the whole thing. Currently the logic flow of the Intro is not smooth: 1. confidence/correctness is different; 2. token activation is important; 3. RAG is challenging; 3. say no when not sure 4. existing method too slow. 5. need to identify source (??) 6. our approach.  I propose to change the logic flow as follows: 1. Principle of abstention is important for FS, thus we quantify uncertainty; 2. It's important to find a way to closely correlate confidence with correctness, especially for RAG, 3. Token activation seems promising, 4. but existing methods are too slow; 5. our approach}



Uncertainty estimation and correctness, while related, are fundamentally orthogonal concepts. A model's high confidence in its output does not necessarily imply correctness, just as a correct response may be assigned low confidence. This distinction becomes particularly salient in retrieval-augmented generation (RAG) applications, where correctness often hinges on factual grounding rather than surface-level fluency.

Consider, for example, the question: "Which is called the red planet?" Both "Mars is the red planet" and the single-word response "Mars" are acceptable answers. In such cases, correctness is determined by the presence of a key factual token—"Mars"—rather than the surrounding context. The uncertainty associated with generating this critical token, as reflected in its token-level generation probability, serves as a valuable signal for estimating confidence. This insight has been leveraged effectively in prior work, where token-level probabilities have shown predictive power for uncertainty estimation ~\cite{bakman2024mars,liu2024uncertainty, malinin2020uncertainty, kuhn2023semantic}.


While existing approaches to uncertainty estimation in retrieval-augmented generation (RAG) have shown promise, they often fall short when the target response is long and narrative in nature. This challenge becomes especially pronounced in sensitive domains such as finance, where queries can be ambiguous or underspecified. For instance, a question like "What is the deadline to make a payment on Card Type A?" may retrieve multiple similar documents, each corresponding to different subcategories of the card type. In such cases, both the query and the retrieved context exhibit ambiguity, which can propagate through the RAG pipeline. Simply measuring uncertainty based on generated response is insufficient to ensure correctness. 

% But, rejecting i.e. not to respond/deciding not to present the answer after generation, comes with a cost of utility. Having a reasonable rejection ratio and presenting answers with high accuracy is acceptable in risky domains. Giving a wrong answer is more expensive than not giving an answer. 

This challenge necessitates a principle of abstention. In high-stakes applications like financial customer support, it is often more appropriate and more trustworthy for the system to abstain from answering than to risk providing an incorrect response. While rejecting a query reduces the system's immediate utility, it is a necessary trade-off to preserve accuracy and user trust. The guiding principle is that the reputational and financial cost of a wrong answer is significantly greater than the cost of not providing one. 


% Uncertainty quantification has received a lot of attention with the advent of LLMs. Specifically focusing on the token-level sampling to quantify the confusion when the model is generating a response for a given prompt. These methods require multiple generations of response with variations of input, thus increasing the costs and latency in production. When deploying RAG systems at scale, having multiple generations to quantify if the answer generated from context is prohibitively expensive both in terms of compute and latency. 

However, common methods for quantifying uncertainty, such as methods relying on sampling \cite{bakman2024mars}, are less practical at scale. These techniques rely on generating a response multiple times with slight variations to measure the model's consistency, a process that introduces prohibitive computational costs and latency in a production environment. For RAG systems that must serve users in real-time, such multi-generational approaches are not a viable solution.

% When accounting for the source of the error in tightly regulated domains like finance, medicine etc. chances of error from alethic sources is quite rare. The knowledge articles are written to a standard after passing through several legal and expert review to avoid fines/unwarranted consequences for wrong information. The source is more likely epistemic,  coming from model's parametric knowledge picked up either at pretraining or fine-tuning.

To develop a practical solution, it is crucial to identify the primary source of this uncertainty. In highly regulated fields, the error is rarely due to aleatoric uncertainty (randomness inherent in the data), as knowledge bases are typically vetted by legal and subject-matter experts. The more probable source is epistemic uncertainty (the model's own lack of knowledge), which arises when the model's parametric knowledge, acquired during pre-training or fine-tuning, conflicts with or misinterprets the provided context. 

\begin{figure*}[htbp]
\centering
\includegraphics[width=1.0\textwidth]{figs/confidence_score_paper-flow Diagram.png}
\caption{Diagram of the proposed Retrieval Augmented Generation (RAG) with the confidence model. When a user asked a question, the IR component retrieves related context from a database. The prompt is then constructed and sent into a question and answering LLM. A confidence score would be generated by the confidence model and being used to control whether or not to show the result to the user. }
\label{fig:utility}
\end{figure*}

Figure~\ref{fig:utility} illustrates the practical utility of integrating a confidence model into our RAG pipeline. The primary goal of the system is to provide users with accurate answers. However, in cases where there is insufficient epistemic or aleatoric knowledge to reliably answer a question, the system's next best action is to abstain from answering. This behavior is enabled by a controller that filters responses based on their confidence scores, allowing the system to avoid potentially incorrect or misleading outputs. This system is deployed in production to be used at scale, and within a reasonable display rate (Ratio of displayed response to total responses generated by the system), have a high F1 score, and reasonably high Rouge compared to the baseline system without the confidence score filter. Table~\ref{res:best_scores} shows that we achieve a precision $\gt 0.95$  with a masking rate(1 - display rate) of 28.3\%.







